FPT Constant-Approximations for Capacitated Clustering to Minimize the Sum of Cluster Radii

Clustering with capacity constraints is a fundamental problem that attracted significant attention throughout the years. In this paper, we give the first FPT constant-factor approximation algorithm for the problem of clustering points in a general metric into $k$ clusters to minimize the sum of cluster radii, subject to non-uniform hard capacity constraints. In particular, we give a $(15+\epsilon)$-approximation algorithm that runs in $2^{0(k^2\log k)}\cdot n^3$ time. When capacities are uniform, we obtain the following improved approximation bounds: A (4 + $\epsilon$)-approximation with running time $2^{O(k\log(k/\epsilon))}n^3$, which significantly improves over the FPT 28-approximation of Inamdar and Varadarajan [ESA 2020]; a (2 + $\epsilon$)-approximation with running time $2^{O(k/\epsilon^2 \cdot\log(k/\epsilon))}dn^3$ and a $(1+\epsilon)$-approximation with running time $2^{O(kd\log ((k/\epsilon)))}n^{3}$ in the Euclidean space; and a (1 + $\epsilon$)-approximation in the Euclidean space with running time $2^{O(k/\epsilon^2 \cdot\log(k/\epsilon))}dn^3$ if we are allowed to violate the capacities by (1 + $\epsilon$)-factor. We complement this result by showing that there is no (1 + $\epsilon$)-approximation algorithm running in time $f(k)\cdot n^{O(1)}$, if any capacity violation is not allowed.

==> preamble.tex <==
%!TEX root = mainDiskGraphs.tex

\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}

\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{amssymb,amsmath,mathrsfs}
\usepackage{soul}
\usepackage{mathtools}
\usepackage{framed}
\usepackage{mdframed}
\usepackage{tcolorbox}

\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}

\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
\usepackage{todonotes}
\usepackage[linesnumbered, boxed, algosection,noline]{algorithm2e}
\usepackage{graphics}
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
%\usepackage{todonotes}

\newcommand{\OO}{\mathcal{O}}
\newcommand{\cO}{\mathcal{O}}

\usepackage{vmargin}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{redrule}{Reduction Rule}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{reduction}{Reduction Rule}[section]
\newtheorem{conjecture}{Conjecture}[section]

\mathchardef\myhyphen="2D
 
\newcommand{\defparproblem}[4]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
}\vspace{1mm}}

\newcommand{\defproblem}[3]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
}\vspace{1mm}}

\usepackage{booktabs}
\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref}

% general
\newcommand{\yes}{\textsf{Yes}}
\newcommand{\no}{\textsf{No}}
\newcommand{\yesinstance}{\yes-instance}
\newcommand{\noinstance}{\no-instance}
\newcommand{\tw}{\mathtt{tw}}
\newcommand{\equ}{\mathtt{Equiv}}
\newcommand{\NP}{\textsf{NP}}
\newcommand{\coNP}{\textsf{co-NP}}
\newcommand{\FPT}{\textsf{FPT}\xspace}
\newcommand{\XP}{\text{XP}}
\newcommand{\WO}{\textsf{W[1]}}
\newcommand{\WOH}{\textsf{W[1]}-hard}
\newcommand{\WOC}{\textsf{W[1]}-complete}
\newcommand{\WTH}{\textsf{W[2]}-hard}
\newcommand{\WTC}{\textsf{W[2]}-complete}
\newcommand{\NPH}{\textsf{NP}-hard}
\newcommand{\NPC}{\textsf{NP}-complete}
\newcommand{\paraH}{\textsf{para-NP}-hard}
\newcommand{\ETH}{\textsf{ETH}}
\newcommand{\SETH}{\textsf{SETH}}
\newcommand{\alg}{\textsf{ALG}}
\newcommand{\nil}{\ensuremath{\mathtt{nil}}}
\newcommand{\dist}{\ensuremath{\mathsf{dist}}}
\newcommand{\flow}{\ensuremath{\mathsf{Flow}}}
\newcommand{\cupdot}{\mathbin{\mathaccent\cdot\cup}}
\newcommand{\paths}{\mbox{\sf Paths}}

%Problem Name

\usepackage{xspace}
\newcommand{\pname}{\textsc}
\newcommand{\ProblemFormat}[1]{\pname{#1}}
\newcommand{\ProblemIndex}[1]{\index{problem!\ProblemFormat{#1}}}
\newcommand{\ProblemName}[1]{\ProblemFormat{#1}\ProblemIndex{#1}{}\xspace}

\newcommand{\probPVD}{\ProblemName{Planar Vertex Deletion}}
\newcommand{\probCVD}{\ProblemName{Chordal Vertex Deletion}}
\newcommand{\probEB}{\ProblemName{Edge Bipartization}}
\newcommand{\probOCT}{\ProblemName{Odd Cycle Transversal}}
\newcommand{\probEMC}{\ProblemName{Edge Multiway Cut}}
\newcommand{\probGFVS}{\ProblemName{Group Feedback Vertex Set}}
\newcommand{\probEMultiC}{\ProblemName{Edge Multicut}}
\newcommand{\probSFVS}{\ProblemName{Subset Feedback Vertex Set}}
\newcommand{\probTWdel}{\ProblemName{Treewidth-$\eta$ Modulator}}
\newcommand{\probFdel}{\ProblemName{$\mathcal{F}$-Deletion}}
\newcommand{\probFpack}{\ProblemName{$\mathcal{F}$-Packing}}
\newcommand{\probSdel}{\ProblemName{$\mathcal{S}$-Deletion}}
\newcommand{\probSpack}{\ProblemName{$\mathcal{S}$-Packing}}
% Commonly used names
\newcommand{\probVC}{\ProblemName{Vertex Cover}}
\newcommand{\probPlVC}{\ProblemName{Planar Vertex Cover}}
\newcommand{\probPVC}{\ProblemName{Partial Vertex Cover}}
\newcommand{\probPDS}{\ProblemName{Partial Dominating Set}}
\newcommand{\probPrDS}{\ProblemName{Partial $r$-Dominating Set}}
\newcommand{\probFVS}{\ProblemName{Feedback Vertex Set}}
\newcommand{\probIFVS}{\ProblemName{Independent Feedback Vertex Set}}
\newcommand{\probCycPacking}{\ProblemName{Cycle Packing}}
\newcommand{\probPlFVS}{\ProblemName{Planar Feedback Vertex Set}}
\newcommand{\probIS}{\ProblemName{Independent Set}}
\newcommand{\probWIS}{\ProblemName{Weighted Independent Set}}
\newcommand{\probMCIS}{\ProblemName{Multicolored Independent Set}}
\newcommand{\probDS}{\ProblemName{Dominating Set}}
\newcommand{\probrDS}{\ProblemName{$r$-Dominating Set}}
\newcommand{\probrSC}{\ProblemName{$r$-Scattered Set}}
%\newcommand{\probMDS}{\ProblemName{Minimum Dominating Set}}
\newcommand{\probPlDS}{\ProblemName{Planar Dominating Set}}
\newcommand{\probCDS}{\ProblemName{Connected Dominating Set}}
\newcommand{\probDST}{\ProblemName{Dominating Set on Tournaments}}
\newcommand{\probClique}{\ProblemName{Clique}}
\newcommand{\probMC}{\ProblemName{Multicolored Clique}}
\newcommand{\probPClique}{\ProblemName{Partitioned Clique}}
\newcommand{\probqSC}{\ProblemName{$q$-Set Cover}}
\newcommand{\probSC}{\ProblemName{Set Cover}}
\newcommand{\probDSP}{\ProblemName{Dominating Set with Pattern}}
%\newcommand{\probOCT}{\ProblemName{Odd Cycle Transversal}}
%\newcommand{\probEB}{\ProblemName{Edge Bipartization}}
\newcommand{\probHam}{\ProblemName{Hamiltonian Cycle}}
\newcommand{\probPlHam}{\ProblemName{Planar Hamiltonian Cycle}}
\newcommand{\probHamP}{\ProblemName{Hamiltonian Path}}
\newcommand{\probKPath}{\ProblemName{Longest Path}}
\newcommand{\probWKPath}{\ProblemName{Weighted Longest Path}}
\newcommand{\probthreeSAT}{\ProblemName{$3$-SAT}}
\newcommand{\probqSAT}{\ProblemName{$q$-SAT}}
\newcommand{\probcnfSAT}{\ProblemName{CNF-SAT}}
\newcommand{\probthreeCol}{\ProblemName{$3$-Coloring}}
\newcommand{\probqCol}{\ProblemName{$q$-Coloring}}
\newcommand{\probListColoring}{\ProblemName{List Coloring}}
\newcommand{\probOddSet}{\ProblemName{Odd Set}}
\newcommand{\probTuring}{\ProblemName{Short Turing Machine Acceptance}}
\newcommand{\probSI}{\ProblemName{Subgraph Isomorphism}}
\newcommand{\probGI}{\ProblemName{Graph Isomorphism}}
\newcommand{\probWCS}{\ProblemName{Weighted Circuit Satisfiability}}
\newcommand{\probClosestString}{\ProblemName{Closest String}}
\newcommand{\probClosestSubstring}{\ProblemName{Closest Substring}}
\newcommand{\probGridTiling}{\ProblemName{Grid Tiling}}
\newcommand{\probGridTilingLeq}{\ProblemName{Grid Tiling with~$\le$}}
\newcommand{\probUnitDisk}{\ProblemName{Unit Disk Independent Set}}
\newcommand{\probEMWay}{\ProblemName{Edge Multiway Cut}}
\newcommand{\probEDS}{\ProblemName{Edge Dominating Set}}
\newcommand{\probEMWaySets}{\ProblemName{Edge Multiway Cut for Sets}}
\newcommand{\probDirEMWay}{\ProblemName{Directed Edge Multiway Cut}}
\newcommand{\probEMCut}{\ProblemName{Edge Multicut}}
\newcommand{\probMulticut}{\ProblemName{Multicut}}
\newcommand{\probDirEMCut}{\ProblemName{Directed Edge Multicut}}
\newcommand{\probSkewEMCut}{\ProblemName{Skew Edge Multicut}}
\newcommand{\probDFVS}{\ProblemName{Directed Feedback Vertex Set}}
\newcommand{\probDFAS}{\ProblemName{Directed Feedback Arc Set}}
\newcommand{\probDFASC}{\ProblemName{Directed Feedback Arc Set Compression}}
\newcommand{\probPartpq}{\ProblemName{$(p,q)$-Partition}}
\newcommand{\probClusterpq}{\ProblemName{$(p,q)$-Cluster}}
\newcommand{\probSatellite}{\ProblemName{Satellite Problem}}
\newcommand{\probTw}{\ProblemName{Treewidth}}
\newcommand{\probPerfSetMatch}{\ProblemName{Perfect $d$-Set Matching}}
\newcommand{\probHS}{\ProblemName{Hitting Set}}
\newcommand{\probdHS}{\ProblemName{$d$-Hitting Set}}
\newcommand{\probEdHS}{\ProblemName{E$d$-Hitting Set}}
\newcommand{\probSetSplit}{\ProblemName{Set Splitting}}
\newcommand{\probSteiner}{\ProblemName{Steiner Tree}}
\newcommand{\probSteinerF}{\ProblemName{Steiner Forest}}
\newcommand{\probMotif}{\ProblemName{Graph Motif}}
\newcommand{\probColorfulMotif}{\ProblemName{Colorful Graph Motif}}
\newcommand{\probRBDSlong}{\ProblemName{Red-Blue Dominating Set}}
\newcommand{\probRBDS}{\ProblemNameX{RBDS}{Red-Blue Dominating Set}}
\newcommand{\probCRBDSlong}{\ProblemName{Colored Red-Blue Dominating Set}}
\newcommand{\probCRBDS}{\ProblemNameX{Col-RBDS}{Colored Red-Blue Dominating Set}}
\newcommand{\probCVC}{\ProblemName{Connected Vertex Cover}}
\newcommand{\probCFVS}{\ProblemName{Connected Feedback Vertex Set}}
\newcommand{\probCBullHit}{\ProblemName{Connected Bull Hitting}}
\newcommand{\probSetPacking}{\ProblemName{Set Packing}}
\newcommand{\probDisFactors}{\ProblemName{Disjoint Factors}}
\newcommand{\probDisPaths}{\ProblemName{Vertex Disjoint Paths}}
\newcommand{\probChromatic}{\ProblemName{Chromatic Number}}
\newcommand{\probECC}{\ProblemName{Edge Clique Cover}}
\newcommand{\probSubsetSum}{\ProblemName{Subset Sum}}
\newcommand{\probKnapsack}{\ProblemName{Knapsack}}
\newcommand{\probWayCut}{\ProblemName{$s$-Way Cut}}
\newcommand{\probEulerian}{\ProblemName{Eulerian  Deletion}}
\newcommand{\probBisec}{\ProblemName{Minimum Bisection}}
\newcommand{\probMaxBisec}{\ProblemName{Maximum Bisection}}

% specific
\newcommand{\disk}{\ensuremath{\mathsf{disk}}}
\newcommand{\obj}{\ensuremath{\mathsf{obj}}}
\newcommand{\rel}{\ensuremath{\mathsf{relevant}}}
\newcommand{\cri}{\ensuremath{\mathsf{critical}}}
\newcommand{\dis}{\ensuremath{\mathsf{distance}}}
\newcommand{\ft}{\ensuremath{\mathsf{ft}}}
\newcommand{\unc}{\ensuremath{\mathsf{uncontract}}}
\newcommand{\ori}{\ensuremath{\mathsf{origin}}}

